An Event-Based Stack For Data Transmission Through Underwater Multimodal Networks

The DESERT Underwater framework (http://desert-underwater.dei.unipd.it/), originally designed for simulating and testing underwater acoustic networks in sea trials, has recently been extended to support real payload data transmission through underwater multimodal networks. Specifically, the new version of the framework is now able to transmit data in real time through the EvoLogics S2C low-rate and high-rate acoustic modems, the SmartPORT low-cost acoustic underwater modem prototype (AHOI) for IoT applications, as well as Ethernet, surface WiFi, and the BlueComm optical modem. The system can also be tested in the lab by employing a simulated channel, and the EvoLogics S2C DMAC Emulator (DMACE)

==> go <==
#!/bin/bash


if [ $1 = clear ]
then
    rm -f *.aux *.bbl *.blg *.dvi *.log *.ps *.fdb_latexmk *.fff *.fls *.backup *.bak *~
    echo -e "\033[1;34;40m Folder cleaned! \033[0m"
else
    latex $1
    latex $1
    bibtex $1
    bibtex $1
    latex $1
    latex $1

    dvips -D 600 -j0 -Ppdf -G0 -t letter -o $1.ps $1.dvi

    ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $1.ps
fi


